TPP: Transparent Page Placement for CXL-Enabled Tiered-Memory

The increasing demand for memory in hyperscale applications has led to memory becoming a large portion of the overall datacenter spend. The emergence of coherent interfaces like CXL enables main memory expansion and offers an efficient solution to this problem. In such systems, the main memory can constitute different memory technologies with varied characteristics. In this paper, we characterize memory usage patterns of a wide range of datacenter applications across the server fleet of Meta. We, therefore, demonstrate the opportunities to offload colder pages to slower memory tiers for these applications. Without efficient memory management, however, such systems can significantly degrade performance. We propose a novel OS-level application-transparent page placement mechanism (TPP) for CXL-enabled memory. TPP employs a lightweight mechanism to identify and place hot/cold pages to appropriate memory tiers. It enables a proactive page demotion from local memory to CXL-Memory. This technique ensures a memory headroom for new page allocations that are often related to request processing and tend to be short-lived and hot. At the same time, TPP can promptly promote performance-critical hot pages trapped in the slow CXL-Memory to the fast local memory, while minimizing both sampling overhead and unnecessary migrations. TPP works transparently without any application-specific knowledge and can be deployed globally as a kernel release. We evaluate TPP in the production server fleet with early samples of new x86 CPUs with CXL 1.1 support. TPP makes a tiered memory system performant as an ideal baseline (<1% gap) that has all the memory in the local tier. It is 18% better than today's Linux, and 5-17% better than existing solutions including NUMA Balancing and AutoTiering. Most of the TPP patches have been merged in the Linux v5.18 release.

==> bandwidth.tex <==
\section{Page Placement for Bandwidth Expansion}
\label{sec:bandwidth}

Previous sections \S\ref{sec:tpp} and \S\ref{sec:evaluation} have been focusing on the memory capacity-expansion case, where the memory bandwidth provided by \cxlmem is not helpful for overall performance.
Correspondingly, our TPP design descrbied so far aims to minimize the bandwidth consumption from the remote node.
This covers vast majority of \meta's applications, especially considering CPUs with CXL support have all moved to DDR5 which already brings a bandwidth boost in local node.

However, there does exist applications whose performance are constrained by memory bandwidth.
These applications typically perform large data movement.
The data injestion service sitting in front of the AI training cluster is such an example.
To optimize the performance of such applications, the page placement mechanism should allocate some hot pages to the remote node, in order to use the extra bandwidth provided by the \cxlmem.

\paragraph{N:K Skewed Interleave.}
\mosharaf{Consider adding a figure to contrast.}
%\wangh{as mentioned earlier, we make this as a contribution to the bandwidth-expansion use case, which still requires more work to make it transparent that we can claim as future work.}
Existing interleave policy (1:1 interleave) spreads out pages across a set of specified nodes.
When a page allocation request arrives, the target node is selected in a round-robin fashion where each node has the same weight.
Now considering \cxlmem has higher latency and typically lower bandwidth than the local node, this 1:1 interleave is very likely

Upcoming memory controllers enable multiple memory channels per DIMM to support higher memory bandwidth.
In such a system, if the \cxlmem has lower number of memory channels than the top-tier node, the default 1:1 interleave may not allow to fully utilize the available bandwidth of top-tier nodes.
We introduce N:K interleave policy, where every N pages allocated to the top-tier node are followed by K pages allocated to the remote node.
This allocation policy helps arbitrarily set the ratio of a working set across the top-tier and remote nodes, therefore, capitalize the effective bandwidth available to each of the memory nodes.
Current version of TPP allows a user to set N and K based on a workload's bandwidth demand across different memory tiers (by default, N = 1, K = 1).
In future, we want to augment TPP by transparently adjusting N and K during application run-time without any user input. 

\begin{figure}[!t]
	\includegraphics[width=\columnwidth]{plot/nk_interleave}
	\caption{For memory bandwidth-bound application, bandwidth utilization and access latency varies with different interleave ratio.}
	\label{fig:eval-nk_interleave}
\end{figure}

\paragraph{Interleave Policy for Memory Bandwidth Expansion.}
For memory bandwidth-bound applications, CPU to DRAM memory bandwidth often becomes the bottleneck and increases the average memory access latency. 
CXL's additional memory bandwidth can help reduce the latency by spreading memory across the top-tier and remote node. 

To observe the impact of TPP's N:K interleave policy on a memory bandwidth-bound application, we setup \cxlmem to expand the system's memory bandwidth capacity by 40\%.
Remote memory being slow and having lower bandwidth capacity, with Linux's default 1:1 interleave policy,  the application can utilize only 75\% of the system's total bandwidth at a very high tail access latency (Figure~\ref{fig:eval-nk_interleave}). 
For this application, 2:1 interleave policy works the best -- it utilizes 96\% of the available memory bandwidth at the lowest memory access latency.
In this paper, we primarily focus on page placement for CXL-based memory capacity-expansion use case.
We want to explore transparent memory management for memory bandwidth-expansion use case in our future work. 
%\wangh{This is a totally different use case, i.e. bandwidth expansion, I think we put this in a seperate discussion/future-work section. So the paper primarily targets capacity-expansion use case by solving NUMA latency issue; and then we show some work/support for bandwidth-expansion use case.}
%\mosharaf{Sweep over more ratios?}



==> cxl-overview.tex <==
\section{CXL-Memory Overview}

\begin{figure}[!t]
	\centering
	\subfloat[][\textbf{Without CXL}]{
	\label{fig:cxl-less-architecture}
		\includegraphics[width=0.5\columnwidth]{figure/numa-bw-wo-cxl}
	}
	\subfloat[][\textbf{With CXL}]{
	\label{fig:cxl-architecture}
		\includegraphics[width=0.5\columnwidth]{figure/numa-bw-w-cxl}
	}
	\caption{NUMA memory BW/GB ratio is better than existing system}
\end{figure}

\paragraph{CXL Protocols}: 
CXL provides byte addressable memory in the same physical address space and allows transparent memory allocation using standard memory allocation APIs. 
It allows cache-line granularity access to the connected devices; underlying hardware maintains coherency and consistency. 
Bandwidth is like DDR channels; NUMA memory BW/GB ratio is 1.5x better than today’s dual socket systems. 
CXL-Memory access latency is close to NUMA latency on dual socket systems --  it adds ~70-80ns latency over normal DRAM access.
\todo{CXL latency/BW characterization for CPU/FPGA -- load, store, effective BW at different read/write ratio}

\paragraph{Accessibility of CXL Technology}: 
Both Intel and AMD are going to enable CXL support on CPUs starting with Sapphire Rapids (Intel) and Genoa (AMD). 
First generation CPUs with CXL are expected to support CXL.io and CXL.mem protocols while the 2nd generation CXL CPUs are announced to extend the support even for CXL.cache. 
All the tools, drives, and OS changes required to support CXL are open sourced so that anyone can contribute and benefit directly without relying on single supplier solutions.

\paragraph{CXL-Memory Management Challenge}: 
CXL-Memory increases the memory capacity and bandwidth -- but, this does not mean we can arbitrarily put the application working set to CXL-Memory. 

\todo{Use cases where random placement does not benefit: Experiment results of 
\begin{denseitemize} 
	\item Cold file caches absorbing local memory hurts
	\item Anons allocated to remote hursts 
	\item Anon migrated to remote and trapped there hurts
\end{denseitemize}
}


==> default-page-placement.tex <==
\section{Background on Linux Page Placement Policy}
\label{sec:default-linux}
%\mosharaf{I feel like this is too far into the paper to give 1.5 page of background. At the least, compress this.}
%\mosharaf{CPU-less should be highlighted better earlier. It's in section 2, but should be highlighted in intro as well along with the benefits of this on disaggregation.} 

Page management policies of existing Linux kernels are designed assuming that a system will have homogeneous DRAM-only NUMA nodes. 
More importantly, having CPU-less memory nodes changes the locality assumptions (pages accessed by a CPU core needs to be in its local memory node) in existing NUMA memory managements.
In this section, we discuss Linux's shortcomings for tiered memory systems.

\subsection{Page Allocation and Reclamation}
\label{subsec:reclaim}
By default, Linux kernel tries to allocate a page to the memory node local to a CPU where the process is running.
%The page allocator initially tries to get free pages  on the local memory node through a fast path -- hoping there will be no reclamation involved.  
To track whether a node has enough free pages for the allocation, it maintains three watermarks (\texttt{min\_watermark}, \texttt{low\_watermark}, \texttt{high\_watermark}) for each memory zone within that node.
If the total number of free pages for a node goes below \texttt{low\_watermark}, Linux considers the node is under memory pressure and initiates page reclamation for that node~(\circled{1} in Figure~\ref{fig:linux-reclaim}). 
It initially tries to free up inactive file caches.
If that is not enough, it then moves to free up anon and mapped file pages.
At this point, the reclaimer initiates paging mechanism  -- it accesses swapping device to page out the colder memory.
Invoking paging events in the critical path worsens the average page access latency and impacts application performance.
%
\begin{figure}[!t]
	\centering
	\subfloat[][\textbf{Reclamation}]{
	\label{fig:linux-reclaim}
		\includegraphics[width=\columnwidth]{figure/reclaim_default}
	}\\
	\subfloat[][\textbf{NUMA Balancing}]{
	\label{fig:linux-numa-balance}
		\includegraphics[width=\columnwidth]{figure/autonuma}
	}
	\caption{Reclamation and NUMA Balancing in default Linux.}
	\label{fig:tpp-challenge}
\end{figure}
%
In a multiple NUMA node system, during this reclamation process, the page allocator checks next eligible memory nodes to grab free pages and new pages get allocated to the remote CPU's memory node~(\circled{2} in Figure~\ref{fig:linux-reclaim}).
Accessing the pages from the remote memory node causes extra NUMA latency as the remote CPU gets involved in the path. 
%Note that the CPU-to-CPU interconnect (UPI) has lower bandwidth and higher latency than the CPU-to-DRAM interconnects.

%After failed attempts to reach the \texttt{high\_watermark} through reclaiming enough pages in direct reclaim mode or if all the memory nodes are low on free pages, the page allocator falls back to a slower allocation path where \texttt{kswapd} is waken up for every node.
%\texttt{kswapd} is a background thread which continues to reclaim pages until the total number of free pages of a node hit the \texttt{high\_watermark}.
%As soon as \texttt{kswapd} frees up enough memory, it goes to a sleep and new allocation can happen on the respective memory node.
When the reclaimer frees up enough memory to satisfy local memory node's \texttt{high\_watermark}, allocation can happen on the local node again.
Both allocation and reclamation check the \texttt{high\_watermark} to decide on when to allocate new pages and when to stop reclaiming, respectively.
With high allocation rate, reclamation may fail to cope-up as it is slower than allocation.
In such a case, memory retrieved by the reclaimer fills up soon to satisfy allocation requests. 
As a result, local memory allocations halt frequently and degrade application performance.
 
%With high allocation rate, reclamation may fail to cope-up as it often needs to go through page-out operations.
%In such a scenario, memory retrieved by the reclaimer fills up soon. 
%As a result, allocations halt frequently and degrade application performance.

\subsection{NUMA Balancing to Reduce Access Latency}
\label{subsec:autonuma}

%\wangh{I would prefer deleting 2nd part; interconnect contention is not super clear here.}
If pages could be allocated to and accessed from a CPU's local memory nodes, average memory access latencies would be minimum and application performance would be optimal.
%When a CPU accesses `remote' memory node, performance penalty arises due to the higher access latency to that remote NUMA node.  
To minimize the access latency from a CPU's remote memory node, one can use NUMA balancing (also known as AutoNUMA)~\cite{autonuma}, an existing Linux kernel feature, that moves pages to a memory node close to the CPU.
A kernel task routinely samples a subset of each process's allocated memory (by default, 256MB of pages) on each memory node and clears the present bit on their flags.
When a CPU accesses a sampled page~(\circled{1} in Figure~\ref{fig:linux-numa-balance}), a minor page-fault is generated (known as NUMA hint fault). 
In the page-fault handler~(\circled{2} in Figure~\ref{fig:linux-numa-balance}), it records which CPU is trying to access the page. 
Pages that are accessed from a remote CPU are migrated to that CPU's local memory node~(\circled{3} in Figure~\ref{fig:linux-numa-balance}) (known as promotion).
NUMA balancing, however, assumes memory nodes are attached to CPUs, therefore, cannot move pages to a CPU-less node (\eg, \cxlmem).
%For a CPU-less memory node, promotion can happen only one direction -- from the CPU-less memory node to the CPU's local memory node. 
%In such a system, unnecessary sampling and NUMA hint faults will cause extra overheads.

%NUMA balancing promotion is a reactive migration.
%Migration candidates are generated only after a sampled page gets hit from the remote CPU.
%Migration does not take place to target node if the target memory node is already in under pressure.
Before promotion, NUMA balancing checks whether the target node has enough free pages to support (\ie, \texttt{high\_watermark} is satisfied). 
If the target node is under pressure, it avoids migration.
At that point, the benefit of NUMA balancing disappears;  pages remain trapped in the remote memory node and experience extra NUMA latency. 
Hot pages trapped to remote node often worsen the performance.

%\vspace{0.5em}
%\noindent\fbox{%
%    \parbox{0.95\columnwidth}{%
%    \textbf{Takeaway:} Existing paging-based reclamation mechanism does not apply for 100 nanosecond-granular \cxlmem.
%Allocation and reclamation being tightly coupled, restrict both new allocation and promotion to local memory node.
%    }
%}
\paragraph{Takeaway.} Linux uses paging mechanism to move cold pages. 
This is latency-intensive and not appropriate to \cxlmem for main memory expansion.
NUMA balancing uses migration for page movement. 
But, it cannot move pages to a CPU-less memory node. 
Besides, allocation and reclamation being tightly coupled, default Linux fails to maintain a headroom of free pages under memory pressure. 
This restricts both new allocation and promotion to local memory node.

%\mosharaf{It'd be better if this section is a bit more than just background. For example, also showing why default don't work.
%Another option is merging into the next section's first subsection.}
